Carbon-Intelligent Global Routing in Path-Aware Networks

The growing energy consumption of Information and Communication Technology (ICT) has raised concerns about its environmental impact. However, the carbon efficiency of data transmission over the Internet has so far received little attention. This carbon efficiency can be enhanced effectively by sending traffic over carbon-efficient inter-domain paths. However, challenges in estimating and disseminating carbon intensity of inter-domain paths have prevented carbon-aware path selection from becoming a reality. In this paper, we take advantage of path-aware network architectures to overcome these challenges. In particular, we design CIRo, a system for forecasting the carbon intensity of inter-domain paths and disseminating them across the Internet. We implement a proof of concept for CIRo on the codebase of the SCION path-aware Internet architecture and test it on the SCIONLab global research testbed. Further, we demonstrate the potential of CIRo for reducing the carbon footprint of endpoints and end domains through large-scale simulations. We show that CIRo can reduce the carbon intensity of communications by at least 47% for half of the domain pairs and the carbon footprint of Internet usage by at least 50% for 87% of end domains.

==> appendices/electricity-cost-estimate.tex <==
\section{Estimating Electricity Price
for Different Sources}
\label{apdx:electricity-price}

Importantly, ISPs are themselves consumers
in the electricity market. Hence, the 
relevant electricity cost metric for ISPs
is not the generation cost of electricity,
but the retail price (including profit 
margins, taxes and fees). However,
to the best of our knowledge,
retail-price data for different sources
of electricity generation across countries 
is not readily available.
We therefore estimate the retail-price
difference between low-emission and 
high-emission electricity on the basis of both
generation costs and integration costs.

Regarding the generation cost of
electricity, we rely on the
well-established 
\emph{levelized cost of energy (LCOE)},
which allows a limited comparison of
electricity-generation sources with
different cost structures. The basic
idea of the LCOE metric is to divide
the total cost accumulating over the
life cycle of an electricity-generating
system (investment, operation, maintenance,
fuel and decommissioning expenditures)
by its generated electricity
volume, while taking into account
capital costs and discount 
rates~\cite{ueckerdt2013system}.
LCOE estimates depend on the exact
methodology, assumptions and paremeters
used in the analysis. Hence, we
rely on LCOE estimates from multiple
studies, namely the following three:
\begin{itemize}
    \item \textbf{Lazard's Levelized Cost of Energy Analysis - Version 14.0 (2020) \cite{lazard2020levelized}:} This study
    claims global validity and presents
    LCOE estimates in USD/MWh.
    \item \textbf{LCOE Estimates for Renewable Energy by Fraunhofer Institute of Solar Energy Systems (F-ISE, 2018) \cite{kost2018levelized}:} This study
    is based on an analysis of the German
    energy system and presents LCOE estimates
    in EUR/MWh, which have been converted
    with an exchange rate of 1.21 USD/EUR.
    \item \textbf{LCOE Estimates by the Paul Scherrer Institute (PSI, 2017) \cite{bauer2017potentials}:} This study
    is based on an analysis of the Swiss
    energy system (accounting for imports)
    and presents LCOE estimates in CHF/MWh,
    which roughly correspond to LCOE estimates
    in USD/MWh because of long-term parity
    between CHF and USD. While the study
    was published in 2017, it contains
    LCOE predictions for 2020.
\end{itemize}

While LCOE is a helpful basis for
comparison, this metric is not sufficient.
As noted by Joskow~\cite{joskow2011comparing}
and Ueckerdt et al.~\cite{ueckerdt2013system},
the LCOE metric only allows a comparison
of electricity-generating technologies
with respect to their cost, but ignores
the differences in value between different
forms of electricity production. In
particular, variable renewable
energies (VRE), including wind and solar,
have a lower value than conventionally
generated electricity due to their
variability and remote production.
If VRE are integrated into an energy
system, they incur balancing costs
(backup production capacity 
needed to absorb shortfalls from
prediction errors), grid-related
costs (grid upgrades needed to transfer
electricity from remote centers of
VRE production to consumption centers),
and profile costs (inefficiency arising
from discrepancy between production
peaks and consumption 
peaks)~\cite{hirth2015integration}.
These costs depend on the
extent of VRE penetration, as higher
penetration leads to higher variability
and a smaller residual energy system
usable for back-up.
In a meta-review of over 100 studies,
Hirth et al.~\cite{hirth2015integration}
estimate that these different variants
of integration costs sum up to additional
costs of around
30--42 USD/MWh for wind power at a
wind penetration of 30-40\%, while
conventional plants have negligible
integration costs. We assume that
these integration costs are also
valid for solar-based electricity
production. These integration
costs have been added to the analysis
in Table~\ref{tab:lcoe}.

The LCOE overview presented in 
Table~\ref{tab:lcoe}
illustrates that LCOE estimates
vary considerably between studies,
which is due to different
methodologies, geographical contexts,
and publication dates of the studies.
As it is difficult to compare
individual LCOE estimates of
different studies due to differences
in methodology, we calculate
the cost penalty of low-emission
sources of electricity generation
over high-emission sources for
each study separately.
The average of these cost penalties,
which are comparable across studies,
is 1.34, meaning that electricity generation
from low-emission sources is 34\%
more expensive than from high-emission sources.
\begin{table*}[t!]
    \centering
    \caption{Levelized cost of energy (LCOE) for
    different technologies of electricity generation in USD/MWh. LCOE of variable renewable energy (VRE) technologies (solar and wind) are
    extended with integration costs
    according to an estimate by Hirth
    et al.~\cite{hirth2015integration}.}
    \begin{tabular}{c|c|c|c|c}
        \multicolumn{2}{c|}{} & \multicolumn{3}{c}{Study}\\
        \cline{3-5}
        \multicolumn{2}{c|}{Electricity source} & Lazard~\cite{lazard2020levelized} 
        & F-ISE~\cite{kost2018levelized}
        & PSI~\cite{bauer2017potentials}\\
        \toprule \multirow{11}{*}{\textbf{Low-emission}} & Solar (utility) & 
        29 -- 42 & 45 -- 140  & 90 -- 110\\
        \cline{2-5} & \textit{with integration costs}
        & 59 -- 84 & 75 -- 182 & 120 -- 152\\
        \cline{2-5}  & Wind (onshore) &
        26 -- 54 & 48 -- 100 & 40 -- 190\\
        \cline{2-5}  & \textit{with integration costs} &
        56 -- 96 & 78 -- 142 & 70 -- 232\\
        \cline{2-5}  & Wind (offshore) & 86 & 91 -- 167 & 130 -- 250 \\
        \cline{2-5}  & \textit{with integration costs} &
        116 -- 128 & 121 -- 209 & 160 -- 292\\
        \cline{2-5}  & Hydro (large, new) & -- & -- & 141\\
        \cline{2-5} & Hydro (large, amortized) & -- & -- & 50 -- 80\\
        \cline{2-5} & Nuclear (new) & 129 -- 198 & -- & 51 -- 124\\
        \cline{2-5}  & Nuclear (amortized) & 29 & -- & 40 -- 60\\
        \cmidrule{2-5} & \makecell{Average (equally weighted, all)} & 77 & 135 & 122\\
        \midrule \multirow{5}{*}{\textbf{High-emission}} & Coal (new) & 65 -- 159 & 56 -- 119 & 41 -- 84\\
        \cline{2-5} & Coal (amortized) & 41 & -- & --\\
        \cline{2-5} & Gas CC (new) & 44 -- 73 & 94 -- 121 & 111 -- 126\\
        \cline{2-5} & Gas CC (amortized) & 28 & -- & -- \\
        \cmidrule{2-5} & Average (equally weighted, all) & 60 & 98 & 90\\
        \midrule \multicolumn{2}{c|}{\makecell{Generation-cost penalty of low-emission sources\\
        over high-emission sources}} & 1.28 & 1.38 & 1.36\\
        \hline \multicolumn{2}{c|}{\textbf{Average generation-cost penalty}}
        & \multicolumn{3}{c}{1.34}
    \end{tabular}
    \label{tab:lcoe}
\end{table*}  However, as mentioned initially,
the relevant electricity cost for ISPs
is not the generation cost for
electricity providers, but the retail
price charged by these providers.
Since this retail price includes
a considerable technology-independent 
fixed component in addition to the
generation cost, the increase in retail
price for low-emission electricity
should be lower than the corresponding increase
in generation cost.

In order to estimate the non-generation
price component (NGPC) of 
electricity retail prices,
we perform the analysis in
Table~\ref{tab:retail-price}.
In this analysis, we calculate the
average generation cost for
an MWh in the European Union
according to the composition of
the EU electricity sector, 
compare it to the average retail price
per MWh that is charged to
non-household end consumers and 
consider the difference
the NGPC. The result of this
analysis is that a MWh in
the European Union has
an average generation cost 
of around 80 USD, a retail price
of around 180 USD and thus
an average NGPC of around 
100 USD. Hence, generation cost
makes up only 44\% of the
end-consumer price, which
is consistent with another
estimate~\cite{murray2019paradox}.

Finally, we estimate the difference
in electricity retail price 
between low-emission electricity 
and high-emission electricity.
Using the augmented Lazard
estimates (cf. Table~\ref{tab:lcoe})
for generation costs of 77 USD/MWh
and 60 USD/MWh for low-emission
and high-emission electricity, respectively,
we arrive at the following price
ratio assuming a NGPC of 100 USD/MWh:
\begin{equation}
    \frac{77 + 100}{60 + 100} = \frac{177}{160} \approx 1.1
\end{equation}
In the following, we will thus assume
that switching to low-emission electricity
will increase the energy costs of
an ISP by 10\%.
\begin{table*}[t!]
    \centering
    \caption{Estimate of non-generation
    price component (NGPC) in electricity retail prices
    in EU countries in 2019. All cost and
    price values are in USD/MWh. The LCOE values
    for generation cost of different
    technologies are from the Lazard study~\cite{lazard2020levelized}
    (except the hydro LCOE, which is from
    the PSI study~\cite{bauer2017potentials}),
    and include integration costs.
    The data on the composition
    of EU electricity production are from the European Commission~\cite{ec2020generation}
    and the International Energy Agency~\cite{iea2020eugeneration}.
    The retail-price data refer to
    non-household consumers in the European Union~\cite{ec2020prices},
    include all taxes and levies and
    have been converted to USD with
    an exchange rate of 1.21 USD/EUR.}
    \begin{tabular}{c|c|c|c|c|c}
        \makecell{Electricity\\source} & \makecell{LCOE\\(avg)} & \makecell{Share of EU\\
        electricity\\production} & \makecell{Generation cost\\(avg MWh)} & \makecell{
        Retail price\\(avg)} & \makecell{NGPC}\\
        \toprule Solar & 72 & 4.4 & \multirow{6}{*}{80} & \multirow{6}{*}{180} & \multirow{6}{*}{100}\\
        \cline{1-3} Wind & 100 & 13.3 & &\\
        \cline{1-3} Hydro & 103 & 12.3 & &\\
        \cline{1-3} Nuclear & 94 & 26.7 & &\\
        \cline{1-3} Coal & 77 & 21.4 & &\\
        \cline{1-3} Gas & 43 & 21.4 & &\\
    \end{tabular}
    \label{tab:retail-price}
\end{table*}



==> appendices/impact_on_latency.tex <==
\section{Extended discussion: impacts on the network}\label{apdx:impact_on_quality}
 \paragraph{Convergence of the virtuous feedback cycle} \cref{fig:economic-simulation:correlation} (cf.~\Cref{sec:eval_virtuous})
 highlights that the introduction of
 carbon awareness into path discovery
 and path selection leads to a
 \emph{virtuous cycle}: By improving
 their carbon footprint, ISPs can attract
 additional traffic and thereby increase
 their profit. As a result, the offered
 paths become increasingly carbon-neutral: 
 Over the simulation duration, the average green-energy 
 share grows by 6 percentage points,
 the total emissions are reduced by 20\%,
 and the average carbon intensity of forwarding
 is reduced by 13\%. In general, this decarbonization
 process also leads to higher prices for end-host
 service and inter-AS links as the ISPs shift
 their higher energy costs to their customers.
 Because of traffic elasticity 
 (cf.~\cref{eq:market:demand:path}),
 this higher price level causes a slight drop
 in the total traffic volume that is actually
 sent, which explains the difference 
 between the reductions in total
 emissions and carbon intensity. 
 Eventually, the decarbonization process
 should converge when the cost for
 additional green-energy purchases exceeds
 the revenue from additional traffic
 that can be attracted through carbon-footprint
 improvements; however, this convergence point is 
 not reached within the duration of our simulation.




==> estimating_co2.tex <==
\section{Inter-domain carbon-intelligent routing in path-aware networks}
\label{sec:carbon_aware_communication}
%To realize carbon-aware inter-domain communication, we design a system capable of measuring long-term and instantaneous carbon intensity of inter-domain paths, disseminating this information in a scalable fashion, and optimizing path carbon intensity via a carbon-aware routing algorithm. The overview of our system is depicted in~\cref{fig:carbon_aware_communication:overview}. We discuss the three pillars of our carbon-transparency system in~\cref{sec:estimating} (estimation of path carbon intensity), \cref{sec:embeddingCO2} (dissemination of carbon-intensity information), and \cref{sec:constructingGreenPaths} (finding paths with low carbon intensity).


In this section, we first discuss the requirements and challenges associated with carbon-intelligent routing in a path-aware architecture. Then, we provide an overview of methods and systems we design to overcome these challenges

%\begin{figure}
%	\centering
%	\input{images/system-overview}
%	\caption{Overview of carbon-transparency system. An arrow from component~$A$ to component~$B$ indicates that component~$A$ relies on data generated/transferred by component~$B$.}
%	\label{fig:carbon_aware_communication:overview}
%\end{figure}

\subsection{Requirements and challenges}
\label{sec:requirements}
We have identified two requirements for inter-domain carbon-intelligent routing in a path-aware network architecture.


The first requirement is to characterize the carbon intensity of network paths in a quantitative, accurate and reliable manner. This characterization is complex because the carbon intensity of a network path varies over time and depends on the location of all devices on the path, their real-time traffic, and their electricity mix, which in turn depends on the daytime and the weather conditions. An important challenge in satisfying this requirement is the significant contribution of idle (base) power consumption\footnote{Power, which is denoted by $P$, is defined as instantaneous energy consumption, i.e., $P=\frac{dE}{dt}$ in \SI{}{\j\per\s} or \SI{}{\watt}.} (thus, the idle \co{} emission) to the total power consumption (thus, the total \co{} emission) in network devices. This is challenging because the \co{} emissions caused by the idle power consumption cannot be directly attributed to specific traffic flows, 
as idle power is a permanent part of the power consumption. 

%To address this issue,  we derive a model for estimation of the carbon intensity of inter-domain paths. We combine multiple existing models for the electricity consumption of networks, and network devices and take into account the carbon intensity of the used electricity to derive our proposed model.

%The \emph{novelty} of the model we propose in this paper in comparison to already existing models (e.g., the ones mentioned in~\cref{sec:background}) is three fold: 1) our approach estimates the \co{} emission while other approaches estimate electricity consumption, 2) our approach estimates \co{} on a \emph{per path} basis, while others try to estimate the electricity consumption of the whole network, and 3) we try to estimate the intensity of \co{} per amount of traffic, while others try to estimate the whole electricity consumption.

The second requirement is to disseminate the carbon-intensity information of inter-domain paths to all endpoints. Two challenges arise in designing such a dissemination scheme. On the one hand, the carbon intensity of a path is variable and gets outdated frequently. On the other hand, due to the enormous number of inter-domain paths, frequent dissemination of carbon-intensity information path can be overwhelming in terms of communication and computation costs for participating nodes. 

%To address this issue, we design a system that forecasts the carbon intensity of inter-domain paths for a few hours and disseminates this forecast to all endpoints. This system uses our proposed method for estimating the carbon intensity of paths and existing methods for predicting the carbon intensity of the power grid.

%The third requirement is to make sure that endpoints are provided with the greenest paths (among other types of paths) to any destination at any time. The main challenge in satisfying this requirement is that the carbon intensity of paths varies over time such that the greenest path at a given time might be a polluting path after a few hours
%To address this issue, we design a routing algorithm for path-aware networks to optimize paths based on their carbon intensity forecasts.



%\begin{sloppypar}
%As SCION provides endpoints with a wide range of fine-grained inter-domain paths (i.e., at the level of inter-domain interfaces of the outgoing and incoming border routers of two neighboring ASes), and ensures that packets are forwarded on the paths selected by the sender, it provides a concrete foundation for carbon-aware inter-domain communications on which we establish our system.
%\end{sloppypar}

\subsection{System overview}
In this section, we provide an overview of our inter-domain carbon intelligent routing system,~\systemname{}. In designing~\systemname{}, we assume that a path-aware Internet architecture (e.g., SCI\-ON) is already deployed, since~\systemname's main goal is to leverage the opportunities created by a path-aware Internet architecture to enable endpoints to transmit their traffic over greener inter-domain paths.

%An advantage of using SCION is that SCION paths are specified in the granularity of ingress and egress points to/from each AS. This provides more path diversity, thus, more carbon-intensity diversity, and provides more opportunity for carbon-intelligent routing.

Thus, the main task of~\systemname{} is to provide endpoints with information about the carbon intensity of inter-domain paths. To calculate the carbon intensity of each inter-domain path in a reliable and accurate way,~\systemname{} needs the collaboration of all ASes on each inter-domain path. However, ASes are not willing to disclose information about their internal topologies and electricity providers, which are necessary for calculating the carbon intensity of a path. To address this problem, we design~\systemname{} as a distributed system with instances in all participating ASes. Each AS deploys a local instance of~\systemname{} that estimates, forecasts and disseminates the carbon intensity of \emph{intra-domain} paths between their ingress and egress border routers without disclosing detailed information about the AS's topology. The carbon intensity of an inter-domain path could then be calculated by accumulating the carbon intensity over all constituting intra-domain segments, because carbon intensity of network path is an additive property (cf.~\Cref{sec:model}).

 

\systemname{} consists of two subsystems: (1) the carbon-intensity forecasting subsystem, and (2) the (carbon-intensity) information dissemination subsystem. We design these subsystems such that 
their composition satisfies the requirements mentioned in~\Cref{sec:requirements}.

The \emph{forecasting subsystem} computes day-ahead hourly forecast (i.e., forecast for every next 24 hours) about the carbon intensity of inter-domain paths between inter-domain interfaces of every on-path AS and inserts them into a database shared with the dissemination subsystem. It also facilitates scalable dissemination of carbon-intensity information since forecasting eliminates the need for constantly disseminating real-time carbon-intensity information.

The main building block of the forecasting subsystem is the model we propose for the carbon intensity of inter-domain paths (i.e., \co{} mass emitted per unit of traffic being forwarded on a path in \SI{}{\gram\per\bit}) in~\Cref{sec:model}. We derive this model by studying existing models for energy intensity of core networks and core network devices (i.e., their energy consumption per bit of forwarded traffic in \SI{}{{\kilo\watt\hour}\per\bit}) and taking into account $\mathit{CIE}$ (cf.~\Cref{sec:background:forecasting}). 

The \emph{information dissemination subsystem} disseminates the carbon intensity predicted by the forecasting system across the Internet. We design this system as an extension to the control-plane infrastructure of a path-aware Internet architecture. We extend the functionality of the control plane to encode carbon-intensity forecasts within route-advertisement messages. Hence, we minimize standardization effort, and communication and computation overhead of disseminating carbon-intensity information. Furthermore, endpoints receive this information along with paths without any additional query.

\subsection{Modeling the carbon intensity of backbone inter-domain paths}\label{sec:model}
Data transmission over a network path may cause \co{} emission through two levels of indirection: forwarding traffic causes (electrical) energy consumption on network devices, and the electricity used by each device is generated from energy resources in a process that may emit \co{}, depending on the energy resources.

We define the \textbf{C}arbon \textbf{I}ntensity of \textbf{D}ata \textbf{T}ransmission ($\textit{\cidt{}}$ in \SI{}{\gram\per\bit}) over a network path as the \co{} emission that can be attributed to a unit of data for being transmitted over that path. \cidt{} is an additive path property. as energy is an additive quantity.
\begin{sloppypar}
	

\subsubsection{\textbf{Inter-domain \cidt{}}} Using \cidt{}'s additive property, we write the \cidt{} of an inter-domain path (denoted by $\fullpath{}$) as the sum of \cidt{}s of consecutive AS hops it consists of:
\begin{align}
\begin{split}
\label{eq:cidt_inter_domain_path}
        \textit{\cidt{}}_{\fullpath{}} = 
        \sum_{\ashopi{} \in \fullpath{}} \textit{\cidt{}}_{\ashopi{}},
\end{split}	        
\end{align}
where $\ashop{}$ denotes an AS hop on the inter-domain path in the granularity of its inter-domain interfaces. $\ifpair{}$ denotes the ingress and egress interface pair from/to which the inter-domain path enters/exits the AS hop.
\end{sloppypar}

The additive property is essential for distributed functionality of ~\systemname{}:  each~\systemname{}'s instance only need to compute the \cidt{} of paths within one AS without disclosing topology information with external entities.

\Cref{eq:cidt_inter_domain_path} ignores inter-domain \emph{links} connecting the border routers of neighboring ASes in \label{eq:cidt_path_as_sum_of_ases}. That is because such links are either (1) direct links connecting two routers in the same data center, or (2) peerings via IXPs, IXP federations, IXP port resellers, or layer-2 links to an IXP. In the first case, the \cidt{} of the link is included in the \cidt{} of neighboring ASes. In the second case, according to previous studies, IXPs and resellers form SCION ASes~\cite{Krahenbuhl2021deployment}. Thus, they could compute their \cidt{} as a normal AS as proposed in this section.


\ali{One option we have is to shorten this section by immediately writing equation 9 here, and move how we derived it to the appendix}

\subsubsection{\textbf{Per-hop \cidt{}}} An AS may forward traffic on multiple internal paths (e.g., using ECMP). Therefore, we define the \cidt{} of $\ashop{}$ as the mean of \cidt{}s of all active \emph{intra-domain} paths from its ingress interface to its egress interface. We assume uniform distribution of traffic over all active paths. Thus,
\begingroup
\begin{align}
\begin{split}
\label{eq:cidt_each_as}
	 \textit{\cidt{}}_{\ashop{}} = \frac{1}{|\mathcal{P}_{\ifpair{}}|} \sum_{P_{\ifpair{}} \in \mathcal{P}_{\ifpair{}}} \textit{\cidt{}}_{P_{\ifpair{}}},
\end{split}	 
\end{align}
\endgroup
where $P_{\ifpair{}}$ denotes an \emph{intra-domain} path in the AS that connects  interface \textit{ing} to interface \textit{eg}, and $\mathcal{P}_{\ifpair{}}$ denotes the set of all such paths.  

\subsubsection{\textbf{\cidt{} of a single intra-domain path}}The \cidt{} over a network path within an AS is composed of two components: 1) the marginal \cidt{}, which is the result of the actual amount of energy consumed to forward a bit of data over a path, and 2) amortized \cidt{}, which is the result of energy consumed to keep network paths up and running, irrespective of traffic volume over the path. Therefore, 
\begingroup
\begin{align}
\begin{split}
\label{eq:cidt_each_path}
	 \textit{\cidt{}}_{P_{\ifpair{}}} = 
	 \textit{\cidt{}}_{P_{\ifpair{}}}^{\textit{marginal}}+
	 \textit{\cidt{}}_{P_{\ifpair{}}}^{\textit{amortized}}. 
\end{split}	 
\end{align}
\endgroup
Because of the additive property, we can write
\begingroup
\begin{align}
\label{eq:cidt_from_devices}
        \textit{\cidt{}}_{P_{\ifpair{}}} &=
        \sum_{\substack{\textit{D} \in P_{\ifpair{}}}} \textit{\cidt{}}_{D}^{\textit{marginal}} + \textit{\cidt{}}_{D}^{\textit{amortized}},
\end{align}
\endgroup
where $D$ denotes a network device on $P_{\ifpair{}}$. It can be a core router, or a WDM device such as an optical switch, a regenerators, or an amplifiers.
\begin{sloppypar}

\paragraph{\textbf{Marginal CIDT}} For each device $D$, $\textit{\cidt{}}_{D}^{\textit{marginal}}$ is the result of (1) the marginal energy the device consumes to forward one bit of data ($E_{D}$ in \SI{}{{\kilo\watt\hour}\per\bit} or \SI{}{{\kilo\watt}\per\bps}), and (2)~the marginal energy consumption of the device's external cooling and facilities, which is proportional to $E_{D}$~\cite{multilayer}. Thus, the total marginal energy is also proportional  to $E_{D}$ by a constant factor ($\eta_{\textit{D},\text{c}}$) that specifies the power-usage efficiency (PUE)~\cite{green_grid, multilayer}.


 To compute $\textit{\cidt{}}_{D}^{\textit{marginal}}$, we multiply the total marginal energy by the $\mathit{CIE}$ (cf.~\Cref{sec:background:forecasting}) in the location of that device ($\textit{CIE}_{\textit{D}}$). Therefore,
\begingroup
\begin{align}
\label{eq:cidt_marginal}
        \textit{\cidt{}}_{D}^{\textit{marginal}} =
\eta_{\textit{D},\text{c}}\textit{E}_{\textit{D}}  \textit{CIE}_{\textit{D}}.
\end{align}
\endgroup
\end{sloppypar}

An AS either knows the value of $\eta_{\textit{D},\text{c}}$ at each of its points of presence (PoPs), or it can use the typical value of 2~\cite{multilayer}. We also assume that an AS can obtain the instantaneous and predicted values of $\textit{CIE}_{\textit{D}}$ at all its PoP, either directly from electricity company, or from ElectricityMaps~\cite{electricitymaps:2022}, WattTime~\cite{watttime:2022}, or DACF~\cite{Maji:2022:DACF}. 

An AS can compute the $E_{D}$ of its network devices, irrespective of their types, by using the following formula~\cite{EnergyConsumptionModellingofOpticalNetworks}:
\begingroup
\begin{align}
\label{eq:marginal_energy}
        E_D = \frac{P_{D, \mathit{max}} - P_{D, \mathit{idle}}}{C_{D, \mathit{max}}},
\end{align}
\endgroup
where $P_{D, \mathit{max}}$ is the maximum power consumption of the device (in \SI{}{\kilo\watt}), $P_{D, \mathit{idle}}$ is its idle power consumption (in \SI{}{\kilo\watt}), and $C_{D, \mathit{max}}$ is its maximum capacity (in \SI{}{\bps}). The values of these variables can be obtained from a device specification.

\paragraph{\textbf{Amortized CIDT}} For each device $D$, $\textit{\cidt{}}_{D}^{\textit{amortized}}$ is the result of (1) the amortized idle energy consumption of the device ($E_{D, idle}^{\textit{amortized}}$ in \SI{}{{\kilo\watt\hour}\per\bit} or \SI{}{{\kilo\watt}\per\bps}), (2) the amortized energy consumption of cooling and facilities when the device is idle, which is proportional to $E_{D, idle}^{\textit{amortized}}$,  (3) the amortized energy consumption of the redundant device(s) $D^{\prime}$ provisioned to protect the primary device $D$ for reliability ($E_{D^{\prime}, idle}^{\textit{amortized}}$), and (4) the amortized energy consumption of cooling and facilities associated with redundant device(s), which is proportional to $E_{D^{\prime}, idle}^{\textit{amortized}}$. We assume redundant devices are idle and do not forward any traffic. 

%Like in marginal energy consumption, the total amortized energy consumption of primary and redundant devices are proportional to $E_{D, idle}^{\textit{amortized}}$ and $E_{D^{\prime}, idle}^{\textit{amortized}}$ by constant factors of $\eta_{\textit{D},\text{c}}$ and $\eta_{\textit{D}^{\prime},\text{c}}$ respectively. Furthermore, to compute $\textit{\cidt{}}_{D}^{\textit{amortized}}$, the total amotized energy of primary and redundant devices need to be multiplied by the carbon intensity of used electricity mix at their locations.

Like in marginal energy consumption, we can write:
\begingroup
\begin{align}
\begin{split}
\label{eq:cidt_amortized}
        \textit{\cidt{}}_{D}^{\textit{amortized}} &=
\eta_{\textit{D},\text{c}}\textit{E}_{\textit{D}, idle}^{\textit{amortized}}  \textit{CIE}_{\textit{D}} \\
&+ \sum_{\substack{\textit{D}^{\prime} \in \mathcal{RD}}} \eta_{\textit{D}^{\prime},\text{c}}\textit{E}_{\textit{D}^{\prime}, idle}^{\textit{amortized}}  \textit{CIE}_{\textit{D}^{\prime}},
\end{split}
\end{align}
\endgroup
where $\mathcal{RD}$ denotes the set of redundant devices to protect the primary device D. Such devices can be located in a different location from the primary device, therefore, their $CIE$ could be different from primary device's $CIE$.

We propose a method to amortize the idle energy consumption of a device over every bit of data that is crossing the device. To that end, we hold each bit of data accountable for the total \emph{idle} energy consumption of a device during the time interval the device processes that bit of data. The capacity of the device (in \SI{}{\bps}) determines the duration of this interval: On average, processing of a bit on a device takes $\frac{1}{C_{D, \mathit{max}}}$ (in $\frac{\SI{}{\bit}}{\SI{}{\bps}}$ or \SI{}{\s}). Thus, by multiplying idle power consumption of the device to this duration, we arrive at the idle energy consumption of the device during this interval:
\begingroup
\begin{align}
\label{eq:e_idle}
E_{D, \mathit{idle}}^{\textit{amortized}} = \frac{P_{D, \mathit{idle}}}{C_{D, \mathit{max}}}.
\end{align}
\endgroup
For redundant devices we use their own $P_{D^{\prime}, \mathit{idle}}$. However, the \emph{primary} device forwards the traffic, the processing time is still determined by the maximum capacity of the \emph{primary} device. Therefore, 
\begingroup
\begin{align}
\label{eq:e_idle_redundant}
E_{D^{\prime}, \mathit{idle}}^{\textit{amortized}} = \frac{P_{D^{\prime}, \mathit{idle}}}{C_{D, \mathit{max}}}.
\end{align}
\endgroup
We assume an AS knows the idle power consumption and maximum capacity of all its devices from their specifications.

\subsubsection{\textbf{Final form of per-hop \cidt{}}} By combining \Crefrange{eq:cidt_each_as}{eq:e_idle_redundant} and simplifying, we arrive at the following formula for the \cidt{} of a path within an AS between a pair of interfaces:

\begingroup
\begin{align}
\begin{split}
\label{eq:cidt_final}
        &\textit{\cidt{}}_{\ashop{}} =
        \frac{1}{|\mathcal{P}_{\ifpair{}}|}
        \sum_{P_{\ifpair{}} \in \mathcal{P}_{\ifpair{}}}
        \sum_{\substack{\textit{D} \in P_{\ifpair{}}}}\\
        &\Bigg(\eta_{\textit{D},\text{c}}\frac{P_{D, \mathit{max}}}{C_{D, \mathit{max}}}\textit{CIE}_{\textit{D}}
        +\sum_{\substack{\textit{D}^{\prime} \in \mathcal{RD}}} \eta_{\textit{D}^{\prime},\text{c}}\frac{P_{D^{\prime}, \mathit{idle}}}{C_{D, \mathit{max}}} \textit{CIE}_{\textit{D}^{\prime}}\Bigg).
\end{split}
\end{align}
\endgroup

In~\Cref{eq:cidt_final}, the only time-variant variable is $CIE$, which depends on availability of renewable electricity, which in turn depends on whether condition, and day or night time.

\subsection{Carbon-intensity forecasting subsystem}\label{sec:forecast}
In every AS participating in~\systemname{}, the forecasting subsystem computes day-ahead hourly \cidt{} forecasts between inter-domain interfaces of the ASes. \ali{Figure X} provides an overview of this subsystem. This subsystem is distributed across participating ASes and each of its instances is administered by one AS. Thus, it does not leak internal information of the AS to any external entity.

\subsubsection{\textbf{Required Inputs}}\label{sec:inputs} Each instance of the forecasting system
 performs its predictions using~\Cref{eq:cidt_final}, requiring the following inputs from the AS it is located in:
\begin{enumerate}
	\item The set of all inter-domain interfaces of the AS, and border routers associated with them. ASes already have this information.
	\item Router-level \emph{intra-domain} paths connecting border routers of the same AS to each other, which are computed by intra-domain routing protocols. An AS already has this information through access to its routers' intra-domain routing information base (RIB).
	\item The locations of all network devices of the AS, including routers, optical switches, amplifiers and regenerators. An AS usually already has this information. However, if an AS leases optical fibers from other companies, it might not know the location of optical devices. In that case, the system uses existing models~\cite{multilayer} for IP over WDM networks to find their approximate locations: optical switches and transponders are co-located with routers, and regenerators and amplifiers are located at \SI{1500}{\kilo\meter} and \SI{80}{\kilo\meter} long intervals, respectively, on the great circle on the earth connecting consecutive routers on a path.
	\item Maximum power consumption ($P_{max}$), maximum capacity ($C_{max}$), and idle power consumption ($P_{idle}$) of all network devices in the AS's network. An AS can obtain this information from the specifications of owned devices. However, if this information is not available for primary devices, the forecasting system substitutes $\frac{P_{D, \mathit{max}}}{C_{D, \mathit{max}}}$ 
	(for primary devices) of $\frac{P_{D^{\prime}, \mathit{idle}}}{C_{D, \mathit{max}}}$
	(for redundant devices) in~\Cref{eq:cidt_final} with typical values~\cite{multilayer} for the energy intensity of network devices suggested by existing models for energy consumption of IP over WDM devices. These typical values are available in~\Cref{Tab:energy_intensity}.
	\item The redundant (backup) devices for every network device on the path. An AS already has this information according to their provisioning plans. However, they might not have this information in the optical layer. In such cases, existing models~\cite{multilayer} suggest one redundant device with similar energy intensity to the primary device. To find the locations of redundant optical devices, the system applies the method mentioned in (2).
	\item The PUE at all AS's PoPs, which determines $\eta_{\textit{D},\text{c}}$. If it is not known for some locations, the system uses typical value of 2 proposed by existing models~\cite{multilayer}.
	\item The day-ahead hourly forecast of $CIE$ at all points of presence of the AS, from ElectricityMaps~\cite{electricitymaps:2022}, WattTime~\cite{watttime:2022},~\cite{Maji:2022:DACF}, or electricity companies.
\end{enumerate}
%Note that since the forecasting subsystem is administered by the AS it is located in and does not share this information with external entities, sharing such information with it does not pose any threat to the AS.


\subsubsection{\textbf{Forecasting Procedure}}\label{sec:forecasting_procedure}
This is a periodic procedure that retrieves updated inputs and re-computes day-ahead hourly \cidt{} forecasts for all pairs of interfaces. The periodic re-com\-pu\-ta\-tion is necessary as (1) $\mathit{CIE}$ forecasts are updated with a period of one hour, and (2) paths between inter-domain interfaces could change even  within these 1-hour intervals. Hence, the recomputation is performed
with period~$T = \min(T_{\mathit{CIE}}, T_{\mathit{path}})$, where $T_{\mathit{CIE}}$ is set to 1 hour to retrieve updated $\mathit{C}IE$ forecasts at the beginning of every hour (**:00), and $T_{\mathit{path}}$ is set to collect updated intra-domain RIBs from routers. $T_{\mathit{path}}$ thus depends on the frequency of path changes in an AS and is set by each AS independently.

At each $T_{\mathit{CIE}}$ (i.e., beginning of every hour), the system first retrieves all inputs mentioned in ~\Cref{sec:inputs}. Then, it computes the day-ahead hourly \cidt{} forecast for every pair of inter-domain interfaces on both directions (i.e., both could be ingress or egress interfaces) using~\Cref{eq:cidt_final}. The result for each ingress and egress interface pair is a vector of 24 \cidt{} values associated with the next 24 hours. Finally, the system inserts the results into the \emph{\cidt{} database} shared with the information dissemination subsystem. Each record in the database represents a pair of ingress and egress interfaces. The first two columns store ingress and egress interface, and the next 24 columns store their associated \cidt{} forecast for the next 24 hours. 

At each $T_{\mathit{path}}$, the system compares checks for the change of paths between inter-domain interfaces compared to the previous $T_{\mathit{path}}$. If the path between two interfaces has changed, the system computes the \cidt{} forecast of new path, and updates the database accordingly.

\subsection{Information dissemination subsystem}\label{sec:dissemination}

This (sub)system uses SCION routing infrastructure (i.e., beaconing process) to disseminate \cidt{} forecasts along with path-segment construction by means of the \staticextension{} in PCBs. The benefits of this scheme are three-fold: (1)~low message complexity and communication overhead as it does not send additional messages dedicated to \cidt{}, (2)~low design and implementation effort by re-using existing protocols, and (3)~scalablity to large topologies through SCION's hierarchical routing architecture. However, this hierarchical dissemination only provides \cidt{} forecasts for SCION path segments, and not full paths. Hence, the carbon intensity of intra-AS paths connecting two segments
must be communicated effectively. 

In this section, we first introduce \ciextension{}, a new type of \staticextension{} for PCBs to disseminate \cidt{} forecasts. Then, we explain how ASes use this extension to convey the \cidt{} forecasts of their paths during the beaconing process.

\subsubsection{\textbf{\ciextension{}}} 
\begin{figure}[t]
	\includegraphics[width=\linewidth]{images/CIDTExtension.pdf}
	\caption{\ciextension{} and other PCB fields necessary for CDIT dissemination.}
	\label{fig:cidtextension}
\end{figure}
\Cref{fig:cidtextension} demonstrates the structure of this extension within a PCB. Every AS can include one \ciextension{} in its \asentry{} to disseminate its \cidt{} forecasts. A \ciextension{} is a map from relevant inter-domain interface identifiers (\texttt{IfId}) of the AS to vectors of \cidt{} forecasts. The inclusion of interfaces in the set of relevant interfaces is determined by beaconing type (core or intra-ISD), and whether the AS is initiating the PCB or only propagating it. 

An \texttt{IfId}, as a key of this map, represents the intra-domain segment between the \texttt{IfId} and the egress interface (\texttt{EgIf}) of the \asentry{}. Importantly, the egress interface refers
to the AS egress with respect to \emph{control-plane information dissemination},
not necessarily with respect to the data-plane sending direction. 
Hence, the part of the \texttt{IfId} forecast vector relating to the `forward' path
concerns the intra-AS path from \texttt{IfId} to \texttt{EgIf} ($\textit{\cidt{}}_{\ashopforward{}}$),
whereas the `backward' path leads from  \texttt{EgIf} to \texttt{IfId} ($\textit{\cidt{}}_{\ashopbackward{}}$). Bidirectional forecasts are necessary as SCION paths are reversible while intra-domain paths could be asymmetric.

A \cidt{} forecast vector is a sequence of 48 contiguous unsigned 8-bit integer numbers, each specifying one \cidt{} value in \SI{e-2}{\gram\per\giga\bit}. We choose this unit based on our observation of the \cidt{} range in Internet paths (cf.~\Cref{sec:direct_results}). The first 24 values of the vector represent $\textit{\cidt{}}_{\ashopforward{}}$ forecasts for the 24-hour interval starting from the greatest hour before the PCB's \texttt{TimeStamp}. The second 24 values provide similar information for $\textit{\cidt{}}_{\ashopbackward{}}$. This design ensures time alignment of forecasts added by different ASes at different times.

\subsubsection{\textbf{Timing of \cidt{} dissemination}}
Since \cidt{} forecasts have a 24-hour time window, they need to be disseminated regularly to preserve the temporal continuity of \cidt{} information. This is aligned with the control-plane design of SCION, as PCBs get expired periodically and need to be initiated periodically to preserve connectivity. However, PCBs with \cidt{} forecasts may need a different period than that of ordinary PCBs.

This periodic dissemination, however, does \emph{not} require ASes to have the same frequency or to be synchronized for \cidt{} dissemination. This is due to the time-alignment of all \ciextension{} in a PCB with the PCB's \texttt{timestamp}. This design eliminates the need for collaboration among ASes to synchronize their \cidt{} disseminations. 

Therefore, every AS locally chooses its \cidt{} dissemination period that is between 1 hour to 2.6 hours. We set the lower bound due to the one-hour update period of \cidt{} forecasts by the forecasting subsystem, which makes it unnecessary to disseminate \cidt{} forecasts more than once an hour. We set the upper bound to guarantee the temporal continuity of \cidt{} forecasts on a path segment in the worst case, where all ASes on the path synchronously disseminate PCBs with the same frequency. Such a guarantee is satisfied when the PCB received by the last AS contains valid \cidt{} forecasts for at least one period. This means that this upper bound is $\frac{24}{n-1}$, where $n$ is the number of AS hops on the path segment. Assuming the longest path segment is 10 AS hops long (twice as long as the average AS-hop length in today's Internet\ali{cite}), the upper bound period is 2.6.

\subsubsection{\textbf{The process of \cidt{} dissemination}}
When the beacon service of an AS wants to disseminate \cidt{} forecasts, it first selects a set of received PCBs per origin AS (i.e., PCB initiator). In this selection, a PCB is prioritized
based on its recentness and its share of \texttt{ASEntries} with~\ciextension{}
in order to maximize the temporal and spatial continuity of \cidt{} information.

Then, for each selected PCB and each egress interface (\texttt{EgIf}) to disseminate the PCB to, the beacon service constructs the corresponding \ciextension{}, adds it to the \asentry{}, extends the PCB with the \asentry{} and disseminates it to the egress interface. 

%The content of \ciextension{} depends on the selected PCB's \texttt{Time\-Stamp}, the egress interface (\texttt{EgIf}), and the set of relevant interfaces, which depends on interface the PCB was entered the AS from (i.e., ingress interface or \texttt{IngIf}), the beaconing type, whether the PCB is being initiated or propagated. 

To construct the \ciextension{} for each PCB, the beacon service first queries the \emph{CIDT database} for \cidt{} forecasts between all relevant \texttt{IfId}s and the \texttt{EgIf} in both directions. However, the retrieved results may not be time-aligned with the \texttt{TimeStamp} of the PCB. This is because the database always provides \cidt{} forecasts for the next 24 hours from the current time, but the \ciextension{} have to provide \cidt{} forecast for the next 24 hours after the \texttt{TimeStamp} of the PCB, which is in the past. To solve this problem, it shifts the vector retrieved from the databese to the right by the number of hours past from the \texttt{TimeStamp}'s hour. This way all elements associated with past hours are filled with zeros and forecasts for beyond 24 hours after \texttt{TimeStamp} are eliminated. \simon{The zeroes causes a problem if some end-point uses the forecast vectors as historical data, but I do not know whether we should account for this.	}

\paragraph{\textbf{CIDT dissemination in core beaconing}}
The dissemination subsystem uses core beaconing to disseminate \cidt{} forecasts of core-path segments. For each core PCB that is being disseminated by a core AS, the beacon service constructs a \ciextension{} containing the \cidt{} forecasts only for the intra-domain segment between the ingress and egress interfaces of the PCB. 

Including forecasts for only one interface pair is essential to the scalability of both forecasting
and dissemination in core ASes. This is because core ASes are large ASes with numerous interfaces, so including information about all interfaces of every hop on the path would introduce significant overhead to each PCB. This per-PCB overhead in conjunction with the high message complexity of core beaconing~\cite{Krahenbuhl2021deployment} would hinder scalability. This encoding, however, does not impact the expressiveness of \cidt{} forecasts since each core PCB only specifies one core-path segment and core path segments do not combine with each other.

\paragraph{\textbf{CIDT dissemination in intra-ISD beaconing}}
The forecasting subsystem uses intra-ISD beaconing to disseminate \cidt{} forecasts of up- and down-path segments. Therefore, beacon services include the \cidt{} forecasts between ingress and egress interfaces of disseminated PCBs in \ciextension{}s. However, since an end-to-end path could be a combination of path segments and peering links, it is essential to also provide a \cidt{} forecast of their combination to arrive at the end-to-end \cidt{} forecast. To cover the combination with core-path segments, a core AS originating a non-core PCB includes the \cidt{} forecasts between the \texttt{EgIf} of the PCB and all interfaces connecting to all other core ASes. To cover the combination of up- and down-path segments, any AS disseminating a non-core PCB includes the \cidt{} forecasts between the \texttt{EgIf} of the PCB and all interfaces connecting to all other customer ASes whose \texttt{IfId} is smaller than \texttt{EgIf}. This way, the required information is either encoded in the up-segment or in the down-segment, halving the overhead. To cover the combination of up- or down-path segments with peering links, any AS disseminating a non-core PCB includes the \cidt{} forecasts between the \texttt{EgIf} of the PCB and all interfaces connecting to all peering ASes.

\paragraph{\textbf{Obtaining the \cidt{} of full inter-domain paths}} Once an endpoint retrieves path segments to construct inter-domain path, it computes the \cidt{} of the full path  for the current hour using \ciextension{}s provided by all segments. Note that different path segments have different origination time, and thus their \cidt{} forecast vectors are not necessarily aligned. Therefore, endpoints compute the index of current time for each path segment independently. Then, they accumulate the \cidt{} forecast of all AS hops associated with the current hour to arrive at the \cidt{} of the end-to-end path.






==> makefile <==
FILES = paper
# FILES = $(patsubst %.tex,%,$(wildcard *.tex))
FILES_PDF = $(addsuffix .pdf,$(FILES))
FILES_FINAL_PDF = $(addsuffix -final.pdf,$(FILES))
FILES_DIFF_PDF = $(addsuffix -diff.pdf,$(FILES))

.PHONY: $(FILES_PDF) $(FILES_FINAL_PDF) $(FILES_DIFF_PDF) all clean final diff.pdf

all: $(FILES_PDF) $(FILES_FINAL_PDF)

final: $(FILES_FINAL_PDF)

$(FILES_PDF): %.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape $<

$(FILES_FINAL_PDF): %-final.pdf: %.tex
	latexmk -pdf -jobname=$(basename $@) -bibtex --synctex=1 -shell-escape -pdflatex='pdflatex %O -interaction=nonstopmode -synctex=1 "\newcommand{\final}{}\input{%S}"' $<


P = paper

# default : $P.pdf

# $P.dvi	: $(wildcard *.tex *.bib figures/*.eps)
# 	latex  $P < /dev/null || $(RM) $@
# 	bibtex $P < /dev/null || $(RM) $@
# 	latex  $P < /dev/null || $(RM) $@
# 	latex  $P < /dev/null || $(RM) $@

# $P.pdf  : $(wildcard *.tex *.bib figures/*)
# 	pdflatex --shell-escape $P
# 	bibtex $P
# 	pdflatex --shell-escape $P
# 	pdflatex --shell-escape $P

# $P.ps	: $P.dvi
# 	dvips -tletter -Ppdf $P.dvi -o $P.ps

# $P.ps.gz: $P.ps
# 	$(RM) $P.ps.gz
# 	gzip -9 < $P.ps > $P.ps.gz

# print:	$P.ps

# dist:	$P.ps.gz

clean:
	$(RM) *.log *.aux *.bbl *.blg *.out *.dvi *.ps *.ps.gz *.fdb_latexmk *.synctex.gz *.fls texput.log

